Pillar-based Object Detection for Autonomous Driving

We present a simple and flexible object detection framework optimized for autonomous driving. Building on the observation that point clouds in this application are extremely sparse, we propose a practical pillar-based approach to fix the imbalance issue caused by anchors. In particular, our algorithm incorporates a cylindrical projection into multi-view feature learning, predicts bounding box parameters per pillar rather than per point or per anchor, and includes an aligned pillar-to-point projection module to improve the final prediction. Our anchor-free approach avoids hyperparameter search associated with past methods, simplifying 3D object detection while significantly improving upon state-of-the-art.

==> section/ablation.tex <==
\section{Ablation Study}
\label{sec:ablation}

\subsection{spherical or cylinder view}
\subsection{anchor or no anchor}
\subsection{one stage or two stage}
\subsection{bilinear point unprojection}

==> section/result.tex <==
% \clearpage

\section*{Supplementary Material}
\label{sec:supplement}

\subsection*{Longer training}

\begin{table}[t] 
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\hline
\multirow{2}{*}{Method} & \multicolumn{4}{|c|}{BEV mAP (IoU=0.7)}  & \multicolumn{4}{|c}{3D mAP (IoU=0.7)} \\ 
\cline{2-9}
& Overall  &  0 - 30m  & 30 - 50m & 50m - Inf & Overall & 0 - 30m & 30 - 50m & 50m - Inf \\
\hline
StarNet~\cite{Ngiam2019StarNetTC} (75 epochs) & - & - & - & - & 53.7 & - & - & - \\
\hline
PointPillars$\P$~\cite{Lang_2019_CVPR} & 80.4 & 92.0 & 77.6 & 62.7 & 62.2 & 81.8 & 55.7 & 31.2 \\
\hline
PointPillars$\dag$~\cite{Lang_2019_CVPR} (100 epochs) & 75.57 & 92.1 & 74.06 & 55.47 & 56.62 & 81.01 & 51.75 & 27.94 \\
\hline
MVF~\cite{Zhou2019EndtoEndMF} (100 epochs) & 80.4 & 93.59 & 79.21 & 63.09 & 62.93 & 86.3 & 60.2 & 36.02 \\
\hline
Ours (30 epochs) & \textbf{86.14} & \textbf{95.59} & \textbf{83.62} & \textbf{70.85} & \textbf{67.71} & \textbf{87.46} & \textbf{64.38} & \textbf{39.88} \\\hline
Ours (75 epochs) & \textbf{86.65} & \textbf{95.41} & \textbf{84.51} & \textbf{71.19} & \textbf{69.12} & \textbf{88.26} & \textbf{65.67} & \textbf{41.44} \\
\hline

Improvements (over MVF) & \textbf{+6.25} & \textbf{+1.82} & \textbf{+5.30} & \textbf{+8.1} & \textbf{+6.19} & \textbf{+1.96} & \textbf{+5.47} & \textbf{+5.42} \\
\hline
\bottomrule
\end{tabular}
}
\end{center}
\caption{Results on vehicle\label{table:car2}. $\P$: re-implemented by~\cite{Sun2019ScalabilityIP}, the feature map in the first PointPillars block is two times as big as in others; $\dag$: re-implemented by~\cite{Zhou2019EndtoEndMF}.}
\end{table}

\begin{table}[t] 
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\hline
\multirow{2}{*}{Method} & \multicolumn{4}{|c|}{BEV mAP (IoU=0.7)}  & \multicolumn{4}{|c}{3D mAP (IoU=0.7)} \\ 
\cline{2-9}
& Overall  &  0 - 30m  & 30 - 50m & 50m - Inf & Overall & 0 - 30m & 30 - 50m & 50m - Inf \\
\hline
StarNet~\cite{Ngiam2019StarNetTC} (75 epochs) & - & - & - & - & 66.8 & - & - & - \\
\hline
PointPillars$\P$~\cite{Lang_2019_CVPR}  & 68.7 & 75.0 & 66.6 & 58.7 & 60.0 & 68.9 & 57.6 & 46.0 \\
\hline
PointPillars$\dag$~\cite{Lang_2019_CVPR} (100 epochs) & 68.57 & 75.02 & 67.11 & 53.86 & 59.25 & 67.99 & 57.01 & 41.29 \\
\hline
MVF~\cite{Zhou2019EndtoEndMF} (100 epochs )& 74.38 & 80.01 & 72.98 & 62.51 & 65.33 & 72.51 & 63.35 & 50.62 \\
\hline
Ours (30 epochs) & \textbf{76.45} & \textbf{82.42} & \textbf{74.38} & \textbf{64.91} & \textbf{67.69} & \textbf{75.42} & \textbf{64.88} & \textbf{51.48} \\
\hline
Ours (75 epochs) & \textbf{76.85} & \textbf{82.9} & \textbf{77.15} & \textbf{63.82} & \textbf{70.65} & \textbf{77.87} & \textbf{70.37} & \textbf{54.48} \\
\hline
Improvements (over MVF) & \textbf{+2.47} & \textbf{+2.89} & \textbf{+4.17} & \textbf{+1.31} & \textbf{+5.32} & \textbf{+5.36} & \textbf{+7.02} & \textbf{+3.86} \\
\hline
\bottomrule
\end{tabular}
}
\end{center}
\caption{Results on pedestrian\label{table:ped2}. $\P$: re-implemented by~\cite{Sun2019ScalabilityIP}. $\dag$: re-implemented by~\cite{Zhou2019EndtoEndMF}.}
\end{table}

One recent work~\cite{He2018RethinkingIP} shows object detection models exhibit better performance if it is trained longer. 
%We investigate the performance gap caused by the length of training time and find longer training indeed increases the performance of our model. 
We find the methods we compared to use different training scheduling: StarNet~\cite{Ngiam2019StarNetTC} is trained for 75 epochs; MVF~\cite{Zhou2019EndtoEndMF} and PointPillars~\cite{Lang_2019_CVPR} re-implemented by~\cite{Zhou2019EndtoEndMF} are trained for 100 epochs, while ours in the main text is only trained for 30 epochs. To have a fair comparison to these methods and investigate the effect of training schedule, we report the results of the model trained for 75 epochs. Table~\ref{table:car2} (for vehicles) and Table~\ref{table:ped2} (for pedestrians) show that when being trained longer, the proposed method has additional performance boosting. Also, compared to MVF~\cite{Zhou2019EndtoEndMF} which is trained for 100 epochs, our method improves by 6.19 3D mAP for vehicle and 5.32 3D mAP for pedestrian.  

\subsection*{Parameter Specification}
In this section, we provide details on the parameters of the model. The model consists of  three parts: a multi-view feature learning network; a birds-eye view pillar backbone network; and a detection head. We show the pipeline in Figure~\ref{fig:network:detail} and the additional parameter specification in Table~\ref{table:parameter}. 


\begin{table}[t] 
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c}
\toprule
\hline
\multirow{2}{*}{Stage} & \multicolumn{2}{|c|}{Vehicle Model}  & \multicolumn{2}{|c}{Pedestrian Model}  \\
 \cline{2-5}
 &  Kernel  & Output Size & Kernel & Output Size \\
\hline

\multirow{3}{*}{Multi-view Feature Learning}  &  3x3, 128, stride 1  & 512x512x128 & 3x3, 128, stride 1  & 512x512x128 \\
\cline{2-5}
 &  3x3, 128, stride 2  & 256x256x128 & 3x3, 128, stride 2  & 256x256x128 \\
\cline{2-5}
 &  3x3, 128, stride 2  & 128x128x128 &  3x3, 128, stride 2  & 128x128x128 \\
 
 \hline
 \multirow{2}{*}{Pillar Backbone Block1} &  3x3, 128, stride 2  & 256x256x128 & 3x3, 128, stride 1  & 512x512x128 \\
 \cline{2-5}
 &  \{3x3, 128, stride 1\}x3  & 256x256x128 & \{3x3, 128, stride 1\}x3  & 512x512x128 \\
 
 \hline
  \multirow{2}{*}{Pillar Backbone Block2} &  3x3, 128, stride 1  & 256x256x128 & 3x3, 128, stride 2  & 256x256x128 \\
 \cline{2-5}
 &  \{3x3, 128, stride 1\}x5  & 256x256x128 & \{3x3, 128, stride 1\}x5 & 256x256x128 \\
 
 \hline
   \multirow{2}{*}{Pillar Backbone Block3} &  3x3, 256, stride 2  & 128x128x256 & 3x3, 256, stride 2  & 128x128x256 \\
 \cline{2-5}
 &  \{3x3, 256, stride 1\}x5  & 128x128x256 & \{3x3, 256, stride 1\}x5  & 128x128x256 \\
 \hline
  Detection Head &  \{3x3, 256, stride 1\}x4  & 256x256x256 & \{3x3, 256, stride 1\}x4  & 512x512x256 \\
\hline
\bottomrule
\end{tabular}
}
\end{center}
\caption{Parameters of convolutional kernels and feature map sizes.}
\label{table:parameter}
\end{table}


\begin{figure*}[t]
\centering
    \includegraphics[height=1.35in]{figure/supp-singleview} \\
    (a) Multi-view Feature Learning
    \begin{tabular}{@{}cc@{}}
    \includegraphics[height=1.1in]{figure/supp-pillar}&
    \includegraphics[height=1.1in]{figure/supp-detection} \\
  (b) Pillar Backbone & (c) Detection Head
  \end{tabular}
\caption{Details of the proposed model: (a) the multi-view feature learning module, we show the network for one view; (b) Pillar backbone network; (c) the detection head, we show both the classification network and the regression network. For details on the parameters and the feature map sizes, refer to Table~\ref{table:parameter}.}
\label{fig:network:detail}
\end{figure*}
